Layerwise Proximal Replay: A Proximal Point Method for Online Continual Learning

In online continual learning, a neural network incrementally learns from a non-i.i.d. data stream. Nearly all online continual learning methods employ experience replay to simultaneously prevent catastrophic forgetting and underfitting on past data. Our work demonstrates a limitation of this approach: neural networks trained with experience replay tend to have unstable optimization trajectories, impeding their overall accuracy. Surprisingly, these instabilities persist even when the replay buffer stores all previous training examples, suggesting that this issue is orthogonal to catastrophic forgetting. We minimize these instabilities through a simple modification of the optimization geometry. Our solution, Layerwise Proximal Replay (LPR), balances learning from new and replay data while only allowing for gradual changes in the hidden activation of past data. We demonstrate that LPR consistently improves replay-based online continual learning methods across multiple problem settings, regardless of the amount of available replay memory.

==> sections/method_prev.tex <==
% \section{Layerwise Proximal Replay}

% \begin{figure*}[tp]
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\linewidth]{icml2024/figures/path6.pdf}
%          \caption{}
%          \label{fig:birdview}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=0.45\linewidth]{icml2024/figures/path7.pdf}
%          \caption{}
%          \label{fig:text_birdview}
%      \end{subfigure}
%      \caption{}
% \end{figure*}


% In this section, we introduce Layerwise Proximal Replay (LPR), a simple implementation of the layerwise proximal point method that uses past data hidden activations to guide experience replay's gradient updates.





% \section{Layerwise Proximal Replay}

% \subsection{Notation}

% Let $M = \{M^l\}_{l=1}^L$ be the coreset of past datapoint hidden layers' input activations with $M^l \in \mathbb{R}^{n_l \times d^{l-1}}$ with $n_l$ being the memory size. Let $\boldsymbol{\theta}$ be vectorized and concatenated $\{\theta^l\}_{l=1}^L$ and let $\mathcal{L}_{\tau}(\boldsymbol{\theta}) = \mathcal{L}_{\tau}(\boldsymbol{\theta}; \mathcal{D}_{\tau}, \mathcal{M})$ be our optimization objective, which can be any continual learning objective with experience replay, parameter regularization, etc.

% \subsection{Methodology}
% When presented with the new data batch $\mathcal{D}_{\tau}$, continual learning methods minimize $\mathcal{L}_{\tau}(\boldsymbol{\theta})$ w.r.t. $\boldsymbol{\theta}$. However, naive gradient descent on $\mathcal{L}_{\tau}(\boldsymbol{\theta})$, which sets the parameter update direction to $\nabla\mathcal{L}_{\tau}(\boldsymbol{\theta})$, could lead to catastrophic forgetting of input-output mappings that $f_{\boldsymbol{\theta}}$ learned on $\mathcal{D}_{<\tau}$. We hypothesize that the optimization of $\mathcal{L}_{\tau}(\boldsymbol{\theta})$ that causes less layer-level forgetting can lead to less model-level forgetting. Let $\{\delta_*^l\}_{l=1}^L$ be the parameter update direction of our choice for $\{\theta^l\}_{l=1}^L$ and $\boldsymbol{\delta}_*$ be vectorized and concatenated $\{\delta_*^l\}_{l=1}^L$. We propose the parameter update direction
% \begin{equation}
%     \boldsymbol{\delta}_* = \argmin_{\boldsymbol{\delta}}\ \mathcal{S}(\boldsymbol{\delta}) \label{eq:problem_orig}
% \end{equation}
% where
% \begin{gather}
%     \mathcal{S}(\boldsymbol{\delta}) = \mathcal{L}_{\tau}(\boldsymbol{\theta} + \boldsymbol{\delta}) + \frac{\eta}{2} \sum_{l=1}^L \mathcal{L}_{c}^l(\theta^l,\delta^l,M^l) + ||\delta^l||_2^2, \label{eq:prox_orig}\\
%     \mathcal{L}_{c}^l(\theta, \delta, M) = \mathbb{E}_{m \sim M}  \left[\frac{1}{\sigma_l^2}\lvert\lvert m^{\top}(\theta + \delta) - m^{\top}\theta\rvert\rvert_2^2 \right] \label{eq:regularizer},
% \end{gather}
% $\eta \in \mathbb{R}_{>0}$, $m \in M$ is a past hidden layer activation from a particular layerwise coreset, and $\sigma_l^2 \in (0, \infty)$ is the hyperparameter that controls the stability-plasticity trade-off of $l$-th layer parameters. Intuitively, Equation \ref{eq:problem_orig} determines the parameter update direction $\boldsymbol{\delta}_*$ s.t. $\mathcal{L}_{\tau}$ is minimized, 2-norm of $\boldsymbol{\delta}_*$ is small, and input-output mappings of the linear maps parameterized by $\theta^l+\delta^l$ and $\theta^l$ are not significantly different for datapoints in $M^l$.

% In general, solving Equation \ref{eq:problem_orig} for every gradient descent step is very costly. However, we can instead solve for its approximation where $\mathcal{L}_{\tau}(\boldsymbol{\theta})$ from Equation \ref{eq:prox_orig} is linearized:
% \begin{equation}
%     \mathcal{S}(\boldsymbol{\delta}) \approx \nabla \mathcal{L}_{\tau}(\boldsymbol{\theta})^{\top}\boldsymbol{\delta} + \frac{\eta}{2} \sum_{l=1}^L \mathcal{L}_{c}^l(\theta^l,\delta^l,M^l) + ||\delta^l||_2^2. \label{eq:prox_approx}
% \end{equation}
% As an aside, as $\sigma_l^2 \rightarrow 0$ for all $l$, $\boldsymbol{\delta}_* \rightarrow \nabla \mathcal{L}_{\tau}(\boldsymbol{\theta})$ and we recover vanilla gradient descent on $\mathcal{L}_{\tau}(\boldsymbol{\theta})$. This follows from the proximal perspective of gradient descent.

% We show in the appendix that the solution to Equation \ref{eq:problem_orig} after this approximation can be analytically written as $\boldsymbol{\delta}_* = \{\delta_*^l\}_{l=1}^L$ where
% \begin{align}
%     \delta_*^l = \frac{1}{\eta}\left(\frac{\tp{M^l}M^l}{ n_l \sigma_l^2} + I\right)^{-1} \nabla_{\theta^l} \mathcal{L}_{\tau}(\boldsymbol{\theta})
% \end{align}
% and $\nabla_{\theta^l} \mathcal{L}_{\tau}(\boldsymbol{\theta})$ is the gradient of $\mathcal{L}_{\tau}(\boldsymbol{\theta})$ w.r.t. $\theta^l$.

% LPR updates its model parameters $\boldsymbol{\theta}$ by repeatedly taking gradient descent steps with descent direction $\boldsymbol{\delta}_*$ and step size $\alpha$ ($\eta$ is absorbed into $\alpha$). In addition, while there are many ways to construct the layerwise coresets $M$, we choose to periodically reset $M$ to the hidden activations generated by the feedforward pass of $\mathcal{M}$'s contents through the current timestep neural network. Algorithm \ref{alg:algorithm} illustrates this procedure in detail.
% \begin{algorithm}[tb]
%    \caption{Layerwise Proximal Replay (LPR)}
%    \label{alg:algorithm}
%     \begin{algorithmic}
%         \STATE {\bfseries Input:} network parameters $\boldsymbol{\theta}$, learning rate $\eta$, per batch gradient steps count $S$, preconditioner update interval $T$, stability hyperparameter $\omega^l$, effective memory size $n^l$.
%         \STATE {\bfseries Output:} trained network parameters $\boldsymbol{\theta}$.
%         \\\hrulefill
%         \STATE Initialize the replay buffer: $\mathcal{M} \leftarrow \{\}$.
%         \STATE Initialize the preconditioners $P^l \leftarrow I,\ l \in \{1,...,L\}$.
%         \FOR{$\tau \in \{1,...,\infty\}$}
%             \STATE Obtain the new data batch $\mathcal{D}_{\tau}$.
%             \FOR{$s \in \{1,...,S\}$}
%                 \STATE Compute arbitrary loss $\mathcal{L}_{\tau}(\boldsymbol{\theta})$ using $\mathcal{D}_{\tau}$ and $\mathcal{M}$.
%                 \STATE Compute the loss gradient $\nabla \mathcal{L}_{\tau}(\boldsymbol{\theta})$.
%                 \FOR{layer index $l \in \{1,...,L\}$}
%                     \STATE $\theta^l \leftarrow \theta^l - \eta P^l\nabla_{\theta^l} \mathcal{L}_{\tau}(\boldsymbol{\theta})$
%                 \ENDFOR
%             \ENDFOR
%             \STATE Update $\mathcal{M}$ with $\mathcal{D}_{\tau}$.
%             \IF{$\tau \bmod{T} = 0$}
%                 \STATE Set $Z^1$ to the features $X_{mem} \in \mathbb{R}^{n \times d^1}$ from $\mathcal{M}$.
%                 \FOR{layer index $l \in \{1,...,L\}$}
%                     \STATE Set $c^l$ according to Equation \ref{eq:n_eff}
%                     \STATE $P^l \leftarrow \left(\frac{\omega^l}{c^l n}\tp{Z^l}Z^l + I\right)^{-1}$.
%                     \STATE $Z^{l+1} \leftarrow \phi^{l}(Z^l\theta^l)$.
%                 \ENDFOR
%             \ENDIF
%        \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

